Securing Automotive Architectures with Named Data Networking

As in-vehicle communication becomes more complex, the automotive community is exploring various architectural options such as centralized and zonal architectures for their numerous benefits. Zonal architecture reduces the wiring cost by physically locating related operations and ECUs near their intended functions and the number of physical ECUs through function consolidation. Centralized architectures consolidate the number of ECUs into few, powerful compute units. Common characteristics of these architectures include the need for high-bandwidth communication and security, which have been elusive with standard automotive architectures. Further, as automotive communication technologies evolve, it is also likely that multiple link-layer technologies such as CAN and Automotive Ethernet will co-exist. These alternative architectures promise to integrate these diverse sets of technologies. However, architectures that allow such co-existence have not been adequately explored. In this work we explore a new network architecture called Named Data Networking (NDN) to achieve multiple goals: provide a foundational security infrastructure and bridge different link layer protocols such as CAN, LIN, and automotive Ethernet into a unified communication system. We created a proof-of-concept bench-top testbed using CAN HATS and Raspberry PIs that replay real traffic over CAN and Ethernet to demonstrate how NDN can provide a secure, high-speed bridge between different automotive link layers. We also show how NDN can support communication between centralized or zonal high-power compute components. Security is achieved through digitally signing all Data packets between these components, preventing unauthorized ECUs from injecting arbitrary data into the network. We also demonstrate NDN's ability to prevent DoS and replay attacks between different network segments connected through NDN.

==> notes.tex <==
\section{Related Work}
I foresee this being a discussion focused on automotive Ethernet 

\section{The problems}
\begin{enumerate}
\item support legacy system and new automotive Ethernet segments
\item CAN security does not exist and susceptible to DoS and replay attacks, and we can not implement meaningful security due to lack of space and compute power
\item{vehicle security's necessity - many attack surfaces, so we need to segment different functionality, the industry is approaching this naturally (needs citation)}
%\item{not future proof. (current solutions don't note segmenting the network)}

\item{Traditional approaches adjust the CAN protocol. . . %.that can't scale and 
can not be used for other technologies such as automotive Ethernet (citations) - NDN is acting as a bridge to different technologies}
%. . .can not pracitally be adopted by industry }

\end{enumerate}



\section{The solutions}
\begin{enumerate}
\item ndn naming for replay prevention between segments 
\item ndn signing for authentication
\item ndn naming for signal translation. Names can communicate signal types \item ndn naming for priority. Names can communicate priority 
\item segmenting the network does limit some of CANs ability to mitigate transmission errors and communicate in real time across the network - NDN as a network forwarder between the segments CAN mitigate some of this while implementing security >>
\item ndn caching for error robustness
\item ndn caching for over head elimination. During moments that it is not forwarding requests it can be building packets on the wire and overwriting those of a lower priority / those that are not being used 
\end{enumerate}

\section{limitations of NDN}
\item each network segment is individually vulnerable to internal attacks NOTE that a comuptationally capable computer (pi) between segments allow for 

\section{Why NDN is suited for securing vehicle networks}
I foresee this being a summation of the arguments made in the paper that was written on NDN For automotive security (A Name-Based Secure Communications
Architecture for Vehicular Networks)


\section{Securing CAN messages using NDN}
\subsection{Experimental Attacks}
\subsection{Threat Model}
\subsection{Attacks and Results }
\begin{itemize}
\item{Replay}
\item{DDOS}
\end{itemize}

\section{Testbed description}
\begin{itemize}
\item{Architecture}
\begin{figure}[htbp]
\item{\includegraphics[scale=.3]{NDN-CAN-Diagram.jpg}}
\caption{Network Diagram }
\label{fig}
\end{figure}
\item{Naming}
\begin{enumerate}
    \item {Explanation of how cars naturally send messages}
    \item{How that was emulated in our tests: The used Model}
\end{enumerate}
\end{itemize}


\section{Performance and Security Evaluation}
\begin{itemize}
\item{CAN's Overhead as a base case}
\item{NDN overhead}
\item{Networking overhead}
\item{Signing overhead}
\item{Encryption Overhead}
\item{Argument about how this will decrease in the future as we move away from prototype langue to production langue}
\end{itemize}
\section{Limitations}
Each CAN interface is individually vulnerable to attacks. But the forwarders can detect these (don't know how  . . .yet). Others have attempting this by adjusting the CAN protocol, but we are propose a method that allows the CAN protocol to operate uninhibited with a limited over head imposed by our signing and forwarders.
\section{Future work}
\section{Conclusion}

